Outer Billiards on the Penrose Kite: Compactification and Renormalizaiton

In this long paper we give a fairly complete analysis of outer billiards on the Penrose kite. Our analysis reveals that this 2-dimensional non-compact system has a 3-dimensional compactification, a certain polyhedron exchange map, and that this compactification has a renormalization scheme. These two features allow us to make some sharp statements concerning the distribution, large-scale geometry, fine-scale geometry, and hidden algebraic symmetries of the orbits. For instance, one of our results is that the union of the unbounded orbits has Hausdorff dimension 1. We give a computer-aided proof of the results concerning the compactification and the renormalization. This proof involves finitely many calculations done with exact integer arithmetic.

==> polyA.tex <==


\subsubsection{Layer $1$}


\begin{eqnarray}
\nonumber
A111=\left[\matrix{1&0\cr 1&0\cr 0&0}\right]\left[\matrix{35&-21\cr -20&13\cr 0&0}\right]\left[\matrix{-20&13\cr 14&-8\cr -21&13}\right]\left[\matrix{35&-21\cr -12&8\cr -8&5}\right]\left[\matrix{1&0\cr 1&0\cr -8&5}\right]\left[\matrix{35&-21\cr -20&13\cr -8&5}\right]\\ \nonumber \left[\matrix{-20&13\cr 1&0\cr -8&5}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A112=\left[\matrix{-33&21\cr 22&-13\cr -8&5}\right]\left[\matrix{1&0\cr 1&0\cr -8&5}\right]\left[\matrix{-33&21\cr 14&-8\cr -8&5}\right]\left[\matrix{22&-13\cr 1&0\cr -8&5}\right]\left[\matrix{1&0\cr 1&0\cr 0&0}\right]\left[\matrix{22&-13\cr -7&5\cr 0&0}\right]\\ \nonumber 
\end{eqnarray}

\begin{eqnarray}
\nonumber
A113=\left[\matrix{-33&21\cr 10&-5\cr 0&0}\right]\left[\matrix{-88&55\cr 23&-13\cr 0&0}\right]\left[\matrix{22&-13\cr -3&3\cr -21&13}\right]\left[\matrix{-33&21\cr 52&-31\cr -42&26}\right]\left[\matrix{111&-68\cr -37&24\cr -42&26}\right]\left[\matrix{111&-68\cr -37&24\cr -8&5}\right]\\ \nonumber \left[\matrix{22&-13\cr -3&3\cr -8&5}\right]\left[\matrix{56&-34\cr -3&3\cr -8&5}\right]\left[\matrix{-88&55\cr 31&-18\cr -8&5}\right]\left[\matrix{-33&21\cr 10&-5\cr -8&5}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A114=\left[\matrix{1&0\cr 2&0\cr 13&-8}\right]\left[\matrix{1&0\cr 2&0\cr 0&0}\right]\left[\matrix{22&-13\cr 2&0\cr 0&0}\right]\left[\matrix{-33&21\cr 10&-5\cr -8&5}\right]\left[\matrix{22&-13\cr 10&-5\cr -8&5}\right]\left[\matrix{56&-34\cr -11&8\cr -8&5}\right]\\ \nonumber 
\end{eqnarray}


\subsubsection{Layer $2$}

\begin{eqnarray}
\nonumber
A121=\left[\matrix{35&-21\cr -12&8\cr -8&5}\right]\left[\matrix{1&0\cr 1&0\cr -8&5}\right]\left[\matrix{35&-21\cr -20&13\cr -8&5}\right]\left[\matrix{69&-42\cr -33&21\cr -8&5}\right]\left[\matrix{69&-42\cr -12&8\cr -29&18}\right]\left[\matrix{-20&13\cr 9&-5\cr 5&-3}\right]\\ \nonumber \left[\matrix{-20&13\cr 9&-5\cr -16&10}\right]\left[\matrix{1&0\cr 1&0\cr -16&10}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A122=\left[\matrix{1&0\cr 1&0\cr -16&10}\right]\left[\matrix{-33&21\cr 22&-13\cr -16&10}\right]\left[\matrix{22&-13\cr -12&8\cr 5&-3}\right]\left[\matrix{1&0\cr 1&0\cr -8&5}\right]\left[\matrix{-33&21\cr 22&-13\cr -8&5}\right]\left[\matrix{22&-13\cr 1&0\cr -8&5}\right]\\ \nonumber \left[\matrix{-33&21\cr 14&-8\cr -8&5}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A123=\left[\matrix{-20&13\cr 9&-5\cr -16&10}\right]\left[\matrix{69&-42\cr -12&8\cr -16&10}\right]\left[\matrix{-20&13\cr -12&8\cr 5&-3}\right]\left[\matrix{69&-42\cr -12&8\cr -29&18}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A124=\left[\matrix{48&-29\cr -12&8\cr -16&10}\right]\left[\matrix{69&-42\cr -12&8\cr -16&10}\right]\left[\matrix{-20&13\cr -12&8\cr 5&-3}\right]\left[\matrix{69&-42\cr -12&8\cr -29&18}\right]\left[\matrix{69&-42\cr -33&21\cr -8&5}\right]\left[\matrix{-20&13\cr 1&0\cr -8&5}\right]\\ \nonumber \left[\matrix{48&-29\cr -20&13\cr -8&5}\right]\left[\matrix{69&-42\cr -20&13\cr -8&5}\right]
\end{eqnarray}


\subsubsection{Layer $3$}

\begin{eqnarray}
\nonumber
A131=\left[\matrix{-20&13\cr 14&-8\cr -16&10}\right]\left[\matrix{1&0\cr 1&0\cr -16&10}\right]\left[\matrix{1&0\cr 1&0\cr -3&2}\right]\left[\matrix{-54&34\cr 22&-13\cr -3&2}\right]\left[\matrix{-20&13\cr 1&0\cr -3&2}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A132=\left[\matrix{1&0\cr 1&0\cr -3&2}\right]\left[\matrix{-88&55\cr 56&-34\cr -37&23}\right]\left[\matrix{1&0\cr 1&0\cr -16&10}\right]\left[\matrix{-88&55\cr 35&-21\cr -16&10}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A133=\left[\matrix{-20&13\cr 9&-5\cr -37&23}\right]\left[\matrix{35&-21\cr -12&8\cr -16&10}\right]\left[\matrix{69&-42\cr -12&8\cr -16&10}\right]\left[\matrix{-20&13\cr 9&-5\cr -3&2}\right]\left[\matrix{69&-42\cr -12&8\cr -3&2}\right]\left[\matrix{35&-21\cr -12&8\cr -3&2}\right]\\ \nonumber 
\end{eqnarray}

\begin{eqnarray}
\nonumber
A134=\left[\matrix{69&-42\cr -12&8\cr -16&10}\right]\left[\matrix{-41&26\cr 14&-8\cr -16&10}\right]\left[\matrix{69&-42\cr -12&8\cr -3&2}\right]\left[\matrix{14&-8\cr 1&0\cr -3&2}\right]\left[\matrix{-41&26\cr 1&0\cr -3&2}\right]\left[\matrix{14&-8\cr -12&8\cr -3&2}\right]\\ \nonumber 
\end{eqnarray}




\subsubsection{Layer $4$}

\begin{eqnarray}
\nonumber
A141=\left[\matrix{1&0\cr 1&0\cr -3&2}\right]\left[\matrix{90&-55\cr -54&34\cr 31&-19}\right]\left[\matrix{1&0\cr 1&0\cr 10&-6}\right]\left[\matrix{90&-55\cr -33&21\cr 10&-6}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A142=\left[\matrix{22&-13\cr -12&8\cr 10&-6}\right]\left[\matrix{1&0\cr 1&0\cr 10&-6}\right]\left[\matrix{1&0\cr 1&0\cr -3&2}\right]\left[\matrix{56&-34\cr -20&13\cr -3&2}\right]\left[\matrix{22&-13\cr 1&0\cr -3&2}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A143=\left[\matrix{22&-13\cr -7&5\cr 31&-19}\right]\left[\matrix{-33&21\cr 14&-8\cr 10&-6}\right]\left[\matrix{-67&42\cr 14&-8\cr 10&-6}\right]\left[\matrix{22&-13\cr -7&5\cr -3&2}\right]\left[\matrix{-67&42\cr 14&-8\cr -3&2}\right]\left[\matrix{-33&21\cr 14&-8\cr -3&2}\right]\\ \nonumber 
\end{eqnarray}

\begin{eqnarray}
\nonumber
A144=\left[\matrix{-67&42\cr 14&-8\cr 10&-6}\right]\left[\matrix{43&-26\cr -12&8\cr 10&-6}\right]\left[\matrix{-67&42\cr 14&-8\cr -3&2}\right]\left[\matrix{-12&8\cr 1&0\cr -3&2}\right]\left[\matrix{43&-26\cr 1&0\cr -3&2}\right]\left[\matrix{-12&8\cr 14&-8\cr -3&2}\right]\\ \nonumber 
\end{eqnarray}


\subsubsection{Layer $5$}

\begin{eqnarray}
\nonumber
A151=\left[\matrix{1&0\cr 1&0\cr 10&-6}\right]\left[\matrix{35&-21\cr -20&13\cr 10&-6}\right]\left[\matrix{-20&13\cr 14&-8\cr -11&7}\right]\left[\matrix{1&0\cr 1&0\cr 2&-1}\right]\left[\matrix{35&-21\cr -20&13\cr 2&-1}\right]\left[\matrix{-20&13\cr 1&0\cr 2&-1}\right]\\ \nonumber \left[\matrix{35&-21\cr -12&8\cr 2&-1}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A152=\left[\matrix{-33&21\cr 14&-8\cr 2&-1}\right]\left[\matrix{1&0\cr 1&0\cr 2&-1}\right]\left[\matrix{-33&21\cr 22&-13\cr 2&-1}\right]\left[\matrix{-67&42\cr 35&-21\cr 2&-1}\right]\left[\matrix{-67&42\cr 14&-8\cr 23&-14}\right]\left[\matrix{22&-13\cr -7&5\cr -11&7}\right]\\ \nonumber \left[\matrix{22&-13\cr -7&5\cr 10&-6}\right]\left[\matrix{1&0\cr 1&0\cr 10&-6}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A153=\left[\matrix{22&-13\cr -7&5\cr 10&-6}\right]\left[\matrix{-67&42\cr 14&-8\cr 10&-6}\right]\left[\matrix{22&-13\cr 14&-8\cr -11&7}\right]\left[\matrix{-67&42\cr 14&-8\cr 23&-14}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A154=\left[\matrix{-46&29\cr 14&-8\cr 10&-6}\right]\left[\matrix{-67&42\cr 14&-8\cr 10&-6}\right]\left[\matrix{22&-13\cr 14&-8\cr -11&7}\right]\left[\matrix{-67&42\cr 14&-8\cr 23&-14}\right]\left[\matrix{-67&42\cr 35&-21\cr 2&-1}\right]\left[\matrix{22&-13\cr 1&0\cr 2&-1}\right]\\ \nonumber \left[\matrix{-46&29\cr 22&-13\cr 2&-1}\right]\left[\matrix{-67&42\cr 22&-13\cr 2&-1}\right]
\end{eqnarray}



\subsubsection{Layer $6$}

\begin{eqnarray}
\nonumber
A261=\left[\matrix{-7&5\cr 6&-3\cr 2&-1}\right]\left[\matrix{1&0\cr 1&0\cr 2&-1}\right]\left[\matrix{-7&5\cr 4&-2\cr 2&-1}\right]\left[\matrix{6&-3\cr 1&0\cr 2&-1}\right]\left[\matrix{1&0\cr 1&0\cr 4&-2}\right]\left[\matrix{6&-3\cr -1&1\cr 4&-2}\right]\\ \nonumber 
\end{eqnarray}

\begin{eqnarray}
\nonumber
A262=\left[\matrix{1&0\cr 1&0\cr 4&-2}\right]\left[\matrix{9&-5\cr -4&3\cr 4&-2}\right]\left[\matrix{-4&3\cr 4&-2\cr -1&1}\right]\left[\matrix{9&-5\cr -2&2\cr 2&-1}\right]\left[\matrix{1&0\cr 1&0\cr 2&-1}\right]\left[\matrix{9&-5\cr -4&3\cr 2&-1}\right]\\ \nonumber \left[\matrix{-4&3\cr 1&0\cr 2&-1}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A263=\left[\matrix{-7&5\cr 2&-1\cr 4&-2}\right]\left[\matrix{-20&13\cr 5&-3\cr 4&-2}\right]\left[\matrix{6&-3\cr -1&1\cr -1&1}\right]\left[\matrix{-7&5\cr 12&-7\cr -6&4}\right]\left[\matrix{27&-16\cr -9&6\cr -6&4}\right]\left[\matrix{27&-16\cr -9&6\cr 2&-1}\right]\\ \nonumber \left[\matrix{6&-3\cr -1&1\cr 2&-1}\right]\left[\matrix{14&-8\cr -1&1\cr 2&-1}\right]\left[\matrix{-20&13\cr 7&-4\cr 2&-1}\right]\left[\matrix{-7&5\cr 2&-1\cr 2&-1}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A264=\left[\matrix{1&0\cr 0&0\cr 7&-4}\right]\left[\matrix{1&0\cr 0&0\cr 4&-2}\right]\left[\matrix{6&-3\cr 0&0\cr 4&-2}\right]\left[\matrix{-7&5\cr 2&-1\cr 2&-1}\right]\left[\matrix{6&-3\cr 2&-1\cr 2&-1}\right]\left[\matrix{14&-8\cr -3&2\cr 2&-1}\right]\\ \nonumber 
\end{eqnarray}

\subsubsection{Layer $7$}

\begin{eqnarray}
\nonumber
A311=\left[\matrix{1&0\cr 1&0\cr 4&-2}\right]\left[\matrix{35&-21\cr -20&13\cr 4&-2}\right]\left[\matrix{-20&13\cr 14&-8\cr -17&11}\right]\left[\matrix{35&-21\cr -12&8\cr -4&3}\right]\left[\matrix{1&0\cr 1&0\cr -4&3}\right]\left[\matrix{35&-21\cr -20&13\cr -4&3}\right]\\ \nonumber \left[\matrix{-20&13\cr 1&0\cr -4&3}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A312=\left[\matrix{-33&21\cr 22&-13\cr -4&3}\right]\left[\matrix{1&0\cr 1&0\cr -4&3}\right]\left[\matrix{-33&21\cr 14&-8\cr -4&3}\right]\left[\matrix{22&-13\cr 1&0\cr -4&3}\right]\left[\matrix{1&0\cr 1&0\cr 4&-2}\right]\left[\matrix{22&-13\cr -7&5\cr 4&-2}\right]\\ \nonumber 
\end{eqnarray}

\begin{eqnarray}
\nonumber
A313=\left[\matrix{-33&21\cr 6&-3\cr 4&-2}\right]\left[\matrix{-88&55\cr 19&-11\cr 4&-2}\right]\left[\matrix{22&-13\cr -7&5\cr -17&11}\right]\left[\matrix{-33&21\cr 48&-29\cr -38&24}\right]\left[\matrix{111&-68\cr -41&26\cr -38&24}\right]\left[\matrix{111&-68\cr -41&26\cr -4&3}\right]\\ \nonumber \left[\matrix{22&-13\cr -7&5\cr -4&3}\right]\left[\matrix{56&-34\cr -7&5\cr -4&3}\right]\left[\matrix{-88&55\cr 27&-16\cr -4&3}\right]\left[\matrix{-33&21\cr 6&-3\cr -4&3}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A314=\left[\matrix{1&0\cr 2&0\cr 17&-10}\right]\left[\matrix{1&0\cr 2&0\cr 4&-2}\right]\left[\matrix{22&-13\cr 2&0\cr 4&-2}\right]\left[\matrix{-33&21\cr 10&-5\cr -4&3}\right]\left[\matrix{22&-13\cr 10&-5\cr -4&3}\right]\left[\matrix{56&-34\cr -11&8\cr -4&3}\right]\\ \nonumber 
\end{eqnarray}


\subsubsection{Layer $8$}
\begin{eqnarray}
\nonumber
A321=\left[\matrix{35&-21\cr -12&8\cr -4&3}\right]\left[\matrix{1&0\cr 1&0\cr -4&3}\right]\left[\matrix{35&-21\cr -20&13\cr -4&3}\right]\left[\matrix{69&-42\cr -33&21\cr -4&3}\right]\left[\matrix{69&-42\cr -12&8\cr -25&16}\right]\left[\matrix{-20&13\cr 9&-5\cr 9&-5}\right]\\ \nonumber \left[\matrix{-20&13\cr 9&-5\cr -12&8}\right]\left[\matrix{1&0\cr 1&0\cr -12&8}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A322=\left[\matrix{1&0\cr 1&0\cr -12&8}\right]\left[\matrix{-33&21\cr 22&-13\cr -12&8}\right]\left[\matrix{22&-13\cr -12&8\cr 9&-5}\right]\left[\matrix{1&0\cr 1&0\cr -4&3}\right]\left[\matrix{-33&21\cr 22&-13\cr -4&3}\right]\left[\matrix{22&-13\cr 1&0\cr -4&3}\right]\\ \nonumber \left[\matrix{-33&21\cr 14&-8\cr -4&3}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A323=\left[\matrix{-20&13\cr 9&-5\cr -12&8}\right]\left[\matrix{69&-42\cr -12&8\cr -12&8}\right]\left[\matrix{-20&13\cr -12&8\cr 9&-5}\right]\left[\matrix{69&-42\cr -12&8\cr -25&16}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A324=\left[\matrix{48&-29\cr -12&8\cr -12&8}\right]\left[\matrix{69&-42\cr -12&8\cr -12&8}\right]\left[\matrix{-20&13\cr -12&8\cr 9&-5}\right]\left[\matrix{69&-42\cr -12&8\cr -25&16}\right]\left[\matrix{69&-42\cr -33&21\cr -4&3}\right]\left[\matrix{-20&13\cr 1&0\cr -4&3}\right]\\ \nonumber \left[\matrix{48&-29\cr -20&13\cr -4&3}\right]\left[\matrix{69&-42\cr -20&13\cr -4&3}\right]
\end{eqnarray}



\subsubsection{Layer $9$}

\begin{eqnarray}
\nonumber
A331=\left[\matrix{-20&13\cr 14&-8\cr -12&8}\right]\left[\matrix{1&0\cr 1&0\cr -12&8}\right]\left[\matrix{1&0\cr 1&0\cr 1&0}\right]\left[\matrix{-54&34\cr 22&-13\cr 1&0}\right]\left[\matrix{-20&13\cr 1&0\cr 1&0}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A332=\left[\matrix{1&0\cr 1&0\cr 1&0}\right]\left[\matrix{-88&55\cr 56&-34\cr -33&21}\right]\left[\matrix{1&0\cr 1&0\cr -12&8}\right]\left[\matrix{-88&55\cr 35&-21\cr -12&8}\right]
\end{eqnarray}

\begin{eqnarray}
\nonumber
A333=\left[\matrix{-20&13\cr 9&-5\cr -33&21}\right]\left[\matrix{35&-21\cr -12&8\cr -12&8}\right]\left[\matrix{69&-42\cr -12&8\cr -12&8}\right]\left[\matrix{-20&13\cr 9&-5\cr 1&0}\right]\left[\matrix{69&-42\cr -12&8\cr 1&0}\right]\left[\matrix{35&-21\cr -12&8\cr 1&0}\right]\\ \nonumber 
\end{eqnarray}

\begin{eqnarray}
\nonumber
A334=\left[\matrix{69&-42\cr -12&8\cr -12&8}\right]\left[\matrix{-41&26\cr 14&-8\cr -12&8}\right]\left[\matrix{69&-42\cr -12&8\cr 1&0}\right]\left[\matrix{14&-8\cr 1&0\cr 1&0}\right]\left[\matrix{-41&26\cr 1&0\cr 1&0}\right]\left[\matrix{14&-8\cr -12&8\cr 1&0}\right]\\ \nonumber 
\end{eqnarray}

